Non-Relational Databases on FPGAs: Survey, Design Decisions, Challenges

Non-relational database systems (NRDS), such as graph, document, key-value, and wide-column, have gained much attention in various trending (business) application domains like smart logistics, social network analysis, and medical applications, due to their data model variety and scalability. The broad data variety and sheer size of datasets pose unique challenges for the system design and runtime (incl. power consumption). While CPU performance scaling becomes increasingly more difficult, we argue that NRDS can benefit from adding field programmable gate arrays (FPGAs) as accelerators. However, FPGA-accelerated NRDS have not been systematically studied, yet. To facilitate understanding of this emerging domain, we explore the fit of FPGA acceleration for NRDS with a focus on data model variety. We define the term NRDS class as a group of non-relational database systems supporting the same data model. This survey describes and categorizes the inherent differences and non-trivial trade-offs of relevant NRDS classes as well as their commonalities in the context of common design decisions when building such a system with FPGAs. For example, we found in the literature that for key-value stores the FPGA should be placed into the system as a smart network interface card (SmartNIC) to benefit from direct access of the FPGA to the network. However, more complex data models and processing of other classes (e.g., graph and document) commonly require more elaborate near-data or socket accelerator placements where the FPGA respectively has the only or shared access to main memory. Across the different classes, FPGAs can be used as communication layer or for acceleration of operators and data access. We close with open research and engineering challenges to outline the future of FPGA-accelerated NRDS.

==> includes/implementation_table_old.tex <==
\begin{table*}[t]
\centering
\scriptsize
\begin{tabular}{l p{2.25cm} p{2.25cm} p{3.00cm} p{2.25cm}} %p{1.50cm}
 & Key-value & Document & Graph & Spatial \\ % & Wide-column
 \hline
 \hline
 \textbf{NoSQL -- functional} & & & & \\
 \hline
 Operator	
 &
 Insert \cite{conf/fpl/LiangYKW16}; Hash \cite{conf/hpcc/LiuZJJ19}
 & 
 Filter \cite{conf/fpl/VanderbauwhedeAM09, conf/reconfig/El-HassanI10, conf/hipeac/MoussalliSNT10, conf/icde/MoussalliSNT11, conf/ispass/ChalamalasettiMVWR12, conf/sigmod/TeubnerWN12, journals/tods/TeubnerWN13, journals/sigarch/VanderbauwhedeFCM13, journals/corr/abs-0909-1781}; 
 Parser \cite{conf/fpga/DaiNZ10, conf/fpt/Sidhu13, HuangJWWP14}
 &
 SP \cite{conf/ipps/BondhugulaDFWS06, journals/tjs/MilovanovicMBT07, journals/iet-cdt/JagadeeshSL11, conf/pdpta/TakeiHK14, TakeiHK15, conf/ipps/ZhouCP15, journals/tcas/LeiDLX16};
 BFS \cite{DBLP:conf/fpt/WangJXP10, conf/asap/BetkaouiWTL12, DBLP:conf/fpl/BetkaouiWTL12, conf/ipps/AttiaJTJZ14, DBLP:journals/ieiceee/NiDZLW14, journals/iracst/LeiRG15, DBLP:conf/fpl/UmurogluMJ15, DBLP:conf/fpga/ZhangKL17, DBLP:conf/fpga/ZhangL18, DBLP:conf/dac/FinnertySLL19};
 MM \cite{DBLP:conf/fpga/BestaFBLH19}; 
 PR \cite{DBLP:conf/reconfig/ZhouCP15}; 
 Centrality \cite{conf/fpl/GiefersSP16}
 &
 Geohash \cite{DBLP:conf/fccm/MoussalliSA15, DBLP:conf/fccm/LeeMAS16}; 
 Geometry \cite{DBLP:conf/dagstuhl/Huthmann0SHK10}; 
 FP \cite{conf/fpt/PaschalakisL03, ThakkarE06, conf/asap/KikkeriS07, DBLP:conf/fpt/VenishettiA07, JaiswalC08, DBLP:conf/hpcc/ZhouDLXD08, DBLP:conf/fccm/BachirD10, DBLP:journals/sigarch/BanescuDPT10, conf/ics/DouLWGZS10, JaiswalC11, conf/fpt/Liebig014}; Other \cite{AriasLAJ12}
 \\
 \hline
 Binary representation	& Hash table \cite{conf/fpl/IstvanABV13, conf/ipps/TongZP15, YangKSKP20}; CAM \cite{conf/hoti/LockwoodM15} &  CAM \cite{conf/reconfig/El-HassanI10} & IS \cite{conf/fpl/ChenBCHHWC19, conf/ccgrid/ZhouLGZZLWZCC17, conf/fpga/DaiCWY16, conf/fpga/DaiHCXWY17, conf/ipps/ZhouCP15, conf/sbac-pad/ZhouP17, conf/cf/ZhouKZP18, journals/tpds/ZhouKPSW19}; CSR \cite{conf/ipps/AttiaJTJZ14}; HW mapping \cite{conf/fpga/Huelsbergen00, conf/fpl/MencerHH02}; Other \cite{SklyarovSP06, conf/hpcc/WangHZZPX15, journals/jsa/WangZH16, conf/fpga/KhoramZSL18, conf/bigdataconf/TariqS18, conf/icws/XuWGJLZ18} & \cite{conf/scss/RiceOS07} \\
 \hline
 Queries	&  & Skeleton automata \cite{conf/sigmod/TeubnerWN12, journals/tods/TeubnerWN13}; Other \cite{conf/www/LunterenEBCL04, NieTW10} & Sparse matrix \cite{conf/hpec/SongGLK16}; Other \cite{conf/asap/Kapre15} &  \\
 \hline
 \hline
 \textbf{NoSQL -- non-functional} & & & & \\
 \hline
 Scalability	& Partitioning \cite{journals/pvldb/IstvanSA17}; Other \cite{journals/pvldb/XuLJLHA16, QiuXLYLWYCGLS20} &   \cite{conf/fpl/VanderbauwhedeAM09} & \cite{conf/other/BabbFA96, DBLP:conf/reconfig/AttiaGTJZ15, conf/fpga/DaiHCXWY17} &  \\
 \hline
 Availability	& Replication \cite{journals/pvldb/IstvanSA17}; Other \cite{conf/hotcloud/BlottKLVBI13, conf/fpga/ChalamalasettiLWARM13, conf/heart/ChoiLLCA18} &  &  &  \\
 \hline
 Consistency	& Multi version \cite{conf/fpl/RenLSXQLYWYCH19} &  & Locking \cite{conf/fpga/MaZC17} &  \\
 \hline
 Multi-tenancy  & \cite{conf/fpl/IstvanAS18} & &  &  \\
 \hline
 Security   	&  &  &  &  \\
 \hline
 \hline
 % & & & & & \\
 \textbf{Accelerator design} & & & & \\
 \hline
 Programmability	&  &  & VC \cite{DBLP:conf/fpl/EngelhardtS16, DBLP:conf/isca/OzdalYKAGBO16, DBLP:conf/micro/HamWSSM16, conf/fpga/DaiCWY16, conf/fpga/DaiHCXWY17, DBLP:journals/corr/abs-1806-00751}, (\cite{WeiszNH13, DBLP:conf/fccm/NurvitadhiWWHNH14, DBLP:conf/reconfig/AttiaGTJZ15}); EC \cite{conf/cf/ZhouKZP18, journals/tpds/ZhouKPSW19}; Hybrid \cite{journals/corr/abs-1806-11509}; Template \cite{journals/tcad/AyupovYOKBO18}; Sparse matrix \cite{conf/fccm/DeLorimierKMRERUKD06, conf/fpl/GiefersSP16}; Other \cite{conf/other/BabbFA96, DBLP:conf/ipps/DandalisMP99, DBLP:conf/fpga/OguntebiO16} &  \\
 \hline
 CPU-FPGA collaboration	& \cite{journals/cal/LavasaniAC14, conf/sosp/LiRXLXPCZ17, conf/fpt/QiuLXYW18, conf/icfpt/XieQYW19, QiuXLYLWYCGLS20} &   \cite{conf/fpl/VanderbauwhedeAM09, journals/sigarch/VanderbauwhedeFCM13}	& \cite{conf/fccm/BondhugulaDDFWSS06, journals/iet-cdt/JagadeeshSL11, DBLP:conf/fpl/UmurogluMJ15, DBLP:journals/pvldb/LeeKYCHNNJ17, conf/sbac-pad/ZhouP17, DBLP:conf/fccm/WangHN19} &  \\
 \hline
 Memory access	& Bloom filter \cite{conf/vlsi-dat/ChoC14, conf/fpl/LiangYKW16}; Flash \cite{conf/hotstorage/BlottLKV15, journals/pvldb/XuLJLHA16} Other \cite{conf/fpt/QiuLXYW18} &  Bloom filter \cite{conf/fpl/VanderbauwhedeAM09} & Sort \cite{DBLP:conf/reconfig/ZhouCP15, conf/fccm/ZhouCP16, DBLP:conf/micro/HamWSSM16, DBLP:conf/fpga/ZhangKL17, DBLP:conf/fpga/ZhangL18, DBLP:conf/dac/FinnertySLL19}; Caching \cite{conf/fpga/KhoramZSL18, DBLP:conf/fpga/ShaoLHL019, DBLP:conf/fccm/WangHN19}; Multi channel \cite{DBLP:journals/ieiceee/NiDZLW14, DBLP:conf/dac/FinnertySLL19}; Other \cite{DBLP:conf/fpt/BetkaouiTLP11, conf/asap/BetkaouiWTL12, DBLP:conf/fpl/BetkaouiWTL12, journals/tcas/LeiDLX16, conf/ccgrid/ZhouLGZZLWZCC17, DBLP:conf/islped/YanHLALMDYZF019} & \cite{conf/ics/DouLWGZS10} \\
 \hline
 Performance model & \cite{QiuXLYLWYCGLS20} &  & \cite{conf/ipps/BondhugulaDFWS06, journals/iet-cdt/JagadeeshSL11, DBLP:conf/fpl/EngelhardtHS18, conf/fpga/DaiCWY16, conf/fpga/DaiHCXWY17, DBLP:conf/fpga/ZhangKL17, journals/tcad/AyupovYOKBO18, conf/icws/XuWGJLZ18, DBLP:conf/fpga/ShaoLHL019} &  \\
\end{tabular}
\caption{Proposed implementations by domain and aspect}
\label{tab:implementations}
\end{table*}

\todo[inline]{Labels?}

==> includes/introduction-old-2.tex <==
\section{Introduction}
\label{sec:introduction}

%1. BACKGROUND/Context (general statements)
% \subsection{Background}
%- NoSQL
In the last few years, NoSQL databases have gained much attention. 
When compared to traditional \glspl{rdbms}, they offer non-relational structuring of data and improved scalability, availability and latency. 
To achieve those properties, they relax traditional database constraints (\eg consistency in PACELC-theorem \cite{journals/computer/Abadi12}). 
Big Data, Internet of Things and other trends benefit greatly from the properties of NoSQL databases and have thus driven a diversification in database systems.
Despite the name, NoSQL is not defined by the lack of a structured query language (SQL), but rather a new way of thinking about databases. 
% Traditionally, databases store data as well formed tables, which impose a structure that is defined at initialization. 
% Strong consistency is a key feature of those databases... 
% \emph{Irgendwie wiederhole ich mich hier nur. Ich glaube eine Auflistung von key paradigm shifts ist hilfreich}

\subsection{NoSQL databases and hardware accelerators}
The key paradigm shifts for NoSQL databases is \emph{variety}, including application-specific data structure, no respectively flexible scheme, horizontal scalability with regard to throughput, replication, partitioning, among others, availability, latency, and often a simplified API.
% No/optional schema
% Horizontal Scaleability (throughput, replication, partitioning)
% Availability
% Latency
% (Simple API)
Overall, these shifts have resulted in a wide-spread acceptance of NoSQL in various technology and business application domains. 
\todo[inline]{possibly some example references here}

% This transition is very weak, because cluster computing does not require performance scaling of single machines!

Similar to data management, computer architecture and technology trends also observed a fundamental change over the recent years.
As a result of the end of Dennard scaling \cite{ref}, frequency scaling is no longer possible and therefore performance scaling is mainly based on massive parallelization.
At the same point in time, power consumption of computing systems became a hard constraint and as a result, the energy efficiency of operations such as computations and memory accesses dominates overall performance.
As a result of the end of Dennard scaling, CPU performance scaling is stuttering, and alternative processor architectures are becoming the foundation of continuing performance scaling, as demanded by applications.
One prime example of such a processor alternative are GPUs, which are massively parallel, operating at rather low frequency for energy efficiency reasons, and widely used as accelerators for tasks that are compute or memory intensive.
On the contrary, GPUs are still today substantially limited in a couple of aspects: 
first, their massive parallelism requires memory subsystems that are capable of keeping these multiple thousands of execution units busy, and the required bandwidth often results in technical limitations of memory capacity. 
As a result, GPUs are notoriously short in memory. 
Second, while it is widely known that GPUs require a massive amount of parallelism in the application, to be more exact a large amount of structured parallelism is required. Otherwise, the lack of structure would result in various performance bugs, such as branch divergence, shared memory bank conflicts, and memory coalescing issues.

Another more recently emerging alternative to CPUs are FPGAs, which are reconfigurable devices in which computations are performed using look-up tables (LUTs) and data can be stored locally in so-called block RAMs (BRAM), which are on-chip SRAM structures.
The reconfigurability aspect of FPGAs allows implementing various architectures, which can also be massively parallel.
At the same time, this reconfigurability makes it harder to compare FPGA-based solutions directly.
From a principle point of view, reconfigurability in the form of so-called soft cores comes at a price: from an efficiency point of view, it is always preferable to implement a module as hard core, being optimized from design to implementation for a specific technology.
However, economic reasons as well as the need to adapt to changes in application behavior often prevent relying solely on hard cores.

Compared to GPUs, FPGAs have a couple of similarities but also differences:
they mainly share the aspects of reduced frequency, massive parallelization, and explicit memory hierarchy.
However, they differ in not being constrained to the use as accelerator, but principally can be deployed anywhere in a compute system.
This is in particular important for concepts like near-data processing or processing on the wire, which allow to substantial reduce the amount of data being moved.
Also, while GPUs excel in floating-point performance, FPGAs rather achieve peak performance for integer-based computations.
As a result, FPGAs are being widely used in various applications, including data centers \cite{conf/isca/PutnamCCCCDEFGGHHHHKLLPPSTXB14}, machine learning \cite{conf/fpga/UmurogluFGBLJV17}, and also data management, which is the focus of this survey.

%2. LITERATURE REVIEW (specific statements)
%\subsection{Literature review}
\subsection{Related surveys}

%\begin{itemize}
%\item 	FPGA vs. CPUs/GPUs: earlier restrictions are being addressed \cite{journals/vldb/FangMHLH20}; feasible for problems similar to NoSQL database workloads \cite{journals/corr/abs-1903-06697}; comment on why GPUs are not applicable (\cite{journals/tlsdkcs/BressHSBS14}); FPGAs can be faster than GPUs for databases: \cite{conf/norchip/RoozmehL17}
%\item 	There are surveys on accelerating traditional databases with FPGAs \cite{conf/fpl/PapaphilippouL18, journals/vldb/FangMHLH20, journals/dbsk/BecherGBDGMPSTW18}
%\item 	There are surveys on NoSQL in general \cite{journals/ife/GessertWFR17, journals/csur/DavoudianCL18, conf/pervasive/HanELD11, GajendranS12, journals/asei/HeC15}
%\item 	Especially graph processing on FPGAs as one aspect of NoSQL got attention. \cite{journals/corr/abs-1903-06697, journals/jcst/Gui0HLCL019}.
%		Those surveys are motivated by high performance computing. 
%		The main weakness is that they focus on the functional aspects.
%\end{itemize}

\begin{figure*}
    \centering
    \includegraphics[width=.75\textwidth]{figures/surveys}
    \caption{Existing survey overview and our contribution}
    \label{fig:surveys}
\end{figure*}

\cref{fig:surveys} shows a Venn diagram of topics related to FPGA-accelerated NoSQL systems. 
In principle there are two main axes of subtopics. 
In light grey we show different kinds of acceleration and in grey we show database system types.
As a secondary axis we also show the popular domains of NoSQL systems in dark grey.

We will introduce the surveys for non-accelerated NoSQL systems later, but otherwise not go into detail of this part of the literature, because it is well covered.
Furthermore we will not revisit GPU acceleration (for graph \cite{journals/csur/ShiZZJHLH18}), because we think GPUs suffer from an IO-bottleneck to the CPU in current systems \cite{journals/tlsdkcs/BressHSBS14}, which is being addressed by FPGAs \cite{journals/vldb/FangMHLH20} and their raised flexibility of deployment.
FPGAs have shown potential to outperform GPUs in database systems. \cite{conf/norchip/RoozmehL17}
Thus, we will focus on the FPGA literature in the vertical middle of \cref{fig:surveys}.

Over the history of database systems there was a development from hierarchical/network databases over relational and object-oriented database systems to NoSQL and very recently NewSQL database systems \cite{journals/csur/DavoudianCL18}. 
Hierarchical/network and object-oriented database systems have since lost popularity, but the relational and NoSQL database system literature shows a trend in accelerator usage.
Thus, we will not go into more detail of the literature on hierarchical/network, object-oriented and NewSQL database systems.

In the last two years, there are surveys structuring the field of FPGA-accelerated relational database systems from different perspectives.
In \cite{journals/dbsk/BecherGBDGMPSTW18}, the authors pose the challenge of using the reconfigurability of the FPGA in relational databases.
This results in open questions on exploitation of heterogeneous hardware, query partitioning and dynamic hardware reconfiguration.
Papaphilippou et al. split up the literature into frameworks (\eg Centaur \cite{conf/fccm/OwaidaSKA17} or DoppioDB \cite{conf/sigmod/SidlerIOKA17}) and specialized accelerators for common operators in a relational database.
They also highlight upcoming technologies for attaching FPGAs to main memory (\ie OpenCAPI) as an important development.
The authors of the most recent survey on the topic \cite{journals/vldb/FangMHLH20} name main memory access, programmability and GPUs as the three biggest factors holding back FPGAs in in-memory relational database systems and how this is being addressed recently, preparing the way for FPGAs as popular accelerators.
While NoSQL systems are very different to relational database systems, we still think these broad trends take over to our area of focus.

We will discuss the NoSQL literature and surveys in more detail in \cref{sec:background}.
Especially graph processing on FPGAs as one domain of NoSQL got attention recently. \cite{journals/corr/abs-1903-06697, journals/jcst/Gui0HLCL019} However, while this shows the feasibilty of graph processing on FPGAs, these surveys are motivated by high performance computing and focus on the functional aspects of graph processing. For our survey this literature has to be viewed from a NoSQL standpoint.

%\begin{itemize}
%    \item Accelerating database systems using \glspl{fpga}: A survey \cite{conf/fpl/PapaphilippouL18}
%    \begin{enumerate}
%        \item Challenges: Main memory access and latency
%        \item Splits literature into frameworks (Centaur, DoppioDB, ...) and specialized accelerators (sort, selection, join, string matching, filtering, arithmetic)
%        \item Also talks about upcoming technologies for attaching FPGA to main memory (OpenCAPI)
%    \end{enumerate}
%    \item In-memory database acceleration on \glspl{fpga}: a survey \cite{journals/vldb/FangMHLH20}
%    \begin{enumerate}
%        \item What held back FPGAs (main memory access, programmability, GPUs) and how this is being addressed
%        \item Functional aspects: acceleration of different query operators (streaming, decompression, sorting, join, partitioning)
%        \item Future research questions: database architecture with multiple different computational elements in mind, accelerator design, comparison with GPUs, compilation for FPGAs
%    \end{enumerate}
%    \item Integration of \glspl{fpga} in Database Management Systems: Challenges and Opportunities \cite{journals/dbsk/BecherGBDGMPSTW18}
%    \begin{enumerate}
%        \item Integration of a FPGA into a DB, with consideration of reconfigurability
%        \item Resulting challenges: exploitation of heterogeneous hardware, query partitioning, dynamic hardware reconfiguration
%    \item NoSQL database systems: a survey and decision guidance \cite{journals/ife/GessertWFR17}
%    \begin{enumerate}
%        \item Key-value, document, wide-column
%        \item ``Comparative classification model that relates functional and non-functional requirements to techniques and algorithms employed in NoSQL databases''
%    \end{enumerate}
%    \item A Survey on NoSQL Stores \cite{journals/csur/DavoudianCL18}
%    \begin{enumerate}
%        \item Strong start with timeline
%        \item Key-value, wide-column, document, graph
%        \item Main aspects are consistency, partitioning and CAP
%    \end{enumerate}
%    \item Survey on NoSQL Database \cite{conf/pervasive/HanELD11}
%    \begin{enumerate}
%        \item Key-value, wide-column, document
%        \item CAP
%    \end{enumerate}
%    \item A Survey on NoSQL Databases \cite{GajendranS12}
%    \begin{enumerate}
%        \item Key-value, wide-column, document
%    \end{enumerate}
%    \item Survey on NoSQL database technology \cite{journals/asei/HeC15}
%    \begin{enumerate}
%        \item Key-value, wide-column, document, graph
%    \end{enumerate}
%    \item Graph Processing on \glspl{fpga}: Taxonomy, Survey, Challenges \cite{journals/corr/abs-1903-06697}
%    \item A Survey on Graph Processing Accelerators: Challenges and Opportunities \cite{journals/jcst/Gui0HLCL019}
%    \begin{enumerate}
%        \item CPU: low efficiency (irregularities do not exploit memory- and instruction-level parallelism)
%        \item GPUs: control and memory divergence, load imbalance, unnecessary global memory accesses
%        \item Preprocessing, parallel graph computation, runtime scheduling
%        \item Major challenge: programmability
%        \item Comprehensive list of algorithms
%    \end{enumerate}
%    \item GPU-Accelerated Database Systems: Survey and Open Challenges \cite{conf/adbis/BressHSBS13} \cite{journals/tlsdkcs/BressHSBS14}
%    \item GraphProcessing on GPUs: A Survey \cite{journals/csur/ShiZZJHLH18}
    %\item Big Data Analytics on Modern Hardware Architectures: A Technology Survey \cite{conf/ebiss/SaeckerM12}
%\end{itemize}

The objective of this survey is to fill this gap in the intersection of FPGA and NoSQL literature, looking at all popular domains of NoSQL database systems from an FPGA-acceleration view.

%3. THE NEED FOR THE PRESENT WORK/Gap (what is missing or wrong in the previous work)
%\subsection{Gap}

%To the best of our knowledge there is not survey on improving NoSQL databases by adding FPGAs to the system.
%Recent surveys in adjacent fields of research show the relevance of the topic and how timely it is, but do not address FPGAs in NoSQL database systems.

%\begin{itemize}
%\item There is a lack of looking at the non-functional aspects; we also look at aspects specific to NoSQL databases on FPGAs (More specific than HPC graph processing, in-memory database on FPGAs, NoSQL in general, ...).
%\item Address FPGA placement opportunities
%\item Systematic overview of the current state of related work.
%\end{itemize}

%4. OBJECTIVE OF THE PRESENT WORK/Innovation (be specific!)
%\subsection{Objective}

% Literature overview and discussion: XXXX

%Objectives:\\
%- existing solutions: Analysis of state-of-the-art and trends in the field of NoSQL database systems: XXX\\
%- patterns, design decisions when building a system: Finding patterns regarding use (operators, placement, optimization) to guide the use of FPGAs for new applications.\\
%- gaps, research questions\\

%\todo[inline]{objectives here or inlined somewhere else? out scope, describe in the context of survey diagram}

% Research method - probably very important for IS Journal, but not VLDBJ
\subsection{Research method}
To address these objectives, this survey relies on the design science methodology \cite{DBLP:books/sp/Wieringa14} as a rigid method to collect, summarize and evaluate FPGA-accelerated NoSQL database solutions.
\Cref{fig:methodology} depicts the research method that we applied, and we used to structure in this paper.
\begin{figure*}
    \centering
    \includegraphics[width=0.7\textwidth]{figures/methodology_v3}
    \caption{Research methodology (adapted from \cite{DBLP:books/sp/Wieringa14})}
    % broken, should be: objectives, artifacts, evaluation
    \label{fig:methodology}
\end{figure*}

Our fundamental theory and motivation for this work is: \emph{Existing NoSQL databases do not leverage modern FPGA hardware}, from which we derive \textbf{hypothesis (H1)}, i.e.,\ \emph{existing NoSQL systems are not sufficiently FPGA hardware-accelerated}.
This hypothesis is tested based on an introductory system review in \cref{sec:background}.
Further, we belief that this grounds on missing fundamental research on hardware-accelerated NoSQL databases (cf. \cref{fig:surveys}), which leads us to \textbf{hypothesis (H2)}, i.e.,\ \emph{current research does not sufficiently address NoSQL hardware acceleration}.
We test this hypothesis on another observation artifact, i.e.,\ a systematic literature review in \cref{sec:literature}.
The system review aims at analyzing available NoSQL systems regarding relevant NoSQL system aspects components / architecture and their current state regarding hardware acceleration.
The derived system aspects are then used to guide the systematic literature review.
The review analyses, which types of NoSQL system types have been previously studied in the context of the system aspects and which solutions are provided.
In \textbf{hypothesis (H3)}, we argue that \emph{it is generally unclear how to build or accelerate a NoSQL database with FPGAs}.
To address the detected gaps and missing FPGA-accelerated NoSQL system, we propose new practical pattern categories, on how to build and accelerated NoSQL database or accelerate and existing one.
Finally, resulting research directions are described.

%5. (optional) JUSTIFICATION OR IMPORTANCE OF THE PRESENT SUBJECT

Without such an overview and analysis of patterns, methodologically sound work would have to redo this effort.
We thus hope, that this survey will be of help for new uses of FPGAs in NoSQL environments, proving a helpful guidance and inspiration for different techniques, methods and concepts (placement, architecture, operator offloading, optimizations).

\subsection{Contributions and outline}

This survey makes the following fundamental contributions (formulated in the form of artifacts) to the field of FPGA-accelerated NoSQL systems:

\begin{itemize}
    \item FPGA-accelerated NoSQL system \emph{aspects} resulting from an analysis of existing NoSQL database systems and challenges in accelerator design for data-centric applications.
    \item Short paper summaries (\emph{implementations}), aspect reference table and list of \emph{gaps} resulting from a comprehensive literature search along structured design science approach. resulting in reference list and short paper summaries.
    \item Patternization of literature into \emph{tasks}, \emph{placements}, non-trivial accelerator design decisions and accelerated architecture justification as guidelines to system architects. 
    \item Open research challenges in the field of FPGA-accelerated NoSQL systems, derived from the gaps in the literature.
\end{itemize}

The reader will get a general background on NoSQL systems and FPGAs (\cref{sec:background}), get an introduction to the current state of the art of FPGA-accelerated NoSQL systems (\cref{sec:literature}), learn how to add an FPGA to a NoSQL system (\cref{sec:practitioners_guide}) and understand the open research challenges of the field (\cref{sec:challenges}).

%6. (optional) PREVIEW
% \subsection{Observations and insights}
% \todo[inline]{What will the reader learn?}

The reader will learn:
\begin{itemize}
    \item What are different nosql domains and how do they currently make use of accelerators (\eg scalable key-value solutions were found, but no complete database solution for others)
    \item For which tasks an accelerator can be used? for an educated accelerator usage decision several aspects have to be considered (\eg operator, communication layer, data access acceleration)
    \item Where to place the accelerator? based on newly identified placement patterns (\eg near-data, socket)
    \item Which non-trivial design decisions will become relevant? (\eg for a complete database implementation dynamic queries, design space reduction, memory access are required among other things)
    \item Why is justification in the form of benchmarks difficult, how it is done today? and what is missing for a solution? (\eg list of data sets, benchmarks available)
\end{itemize}

\todo[inline]{Mit theorem definition package arbeiten}

==> includes/introduction-old-3.tex <==
\section{Introduction}
\label{sec:introduction}

%1. BACKGROUND/Context (general statements)
In the last few years, database systems gained \emph{variety} in database models.
A diversification of database models from mostly relational modeling towards more application-specific modeling (\eg graphs, documents, and key-value pairs) of data took place.
When compared to traditional relational database systems, modern systems implementing such data models offer flexible on-the-fly and application-native modeling of data,
This avoids fixed schemas, restricting abstractions and saves resources spent on data transformation.
Additionally, such modern database systems often relax traditional database system constraints (\eg consistency in PACELC-theorem \cite{journals/computer/Abadi12}) to satisfy application requirements like heightened scalability (with regard to \eg throughput, replication and partitioning), availability, latency and often a simplified API.
Big Data, Internet of Things and other trends benefit greatly from these new properties of modern non-relational databases and have thus driven a diversification in database systems. \cite{bigdata, iot}

Even though modern non-relational database systems follow the guiding principle of application specificity, they do not have many commonalities on first sight.
Complex graph query languages (\eg Cypher \cite{cypher}) share little with simple APIs of key-value stores (insert, read, and delete).
Document filtering uses different algorithms than traversal operators on graphs.
However, we think that non-relational database systems share underlying patterns, making it worthwhile to examine them together.
Furthermore, there is a rising trend of providing multiple data models in the same database system (\eg OrientDB with document and graph data models in one system), requiring effective resource sharing through common patterns. \cite{something}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/introduction}
    \caption{Data model types and their relation}
    \label{fig:datamodel}
\end{figure}

\Cref{fig:datamodel} shows important data model types (blue) and how they fall apart into data structure primitives. Key-value stores directly work on key-value pairs through a hash table, while wide-column stores use column and row names as keys and associate them with values. Graph stores build graphs from vertices connected by edges and associate properties with them, while document stores build documents from objects and arrays that refer to properties again. We argue that properties and key-value pairs are fundamentally the same and thus one of the unifying factors of different non-relational data models. Additionally, each store can support simple lookup operations and the more expressive data models (document and graph) support traversals of their structure to find properties. Furthermore, stores and operators generally have associated constrainednesses.

\subsection{FPGA acceleration for non-relational databases}

Similar to the application driven change in database systems, there has been a fundamental change in computer architectures and technology trends based on ever rising performance requirements of applications.
As a result of the end of Dennard scaling \cite{ref}, frequency and therewith performance scaling of CPUs is stuttering.
%Performance gains were found in the massive distribution of workloads to clusters of computers, which hit a power wall recently.
Power consumption of computing systems is now a hard constraint leading to energy efficiency of operations such as computations and memory accesses dominating overall performance.
Thus, new computer architectures such as GPUs and more recently FPGAs are explored for future performance scaling.

GPUs, on the one hand, are massively parallel processors operating at rather low frequency for energy efficiency reasons, widely used as accelerators for tasks that are compute or memory intensive.
However, GPUs are still today substantially limited in a couple of aspects: 
first, their massive parallelism requires memory subsystems that are capable of keeping their multiple thousands of execution units busy, and the required bandwidth often results in technical limitations of memory capacity. 
As a result, GPUs are notoriously short in memory. 
Second, while it is widely known that GPUs require a massive amount of parallelism in the application, to be more exact a large amount of structured parallelism is required. 
Otherwise, the lack of structure would result in various performance bugs, such as branch divergence, shared memory bank conflicts, and memory coalescing issues.

FPGAs, on the other hand, are reconfigurable processors in which computations are performed using several hundreds of thousand look-up tables (LUTs) and data can be stored locally in so-called block RAMs (BRAM), which are on-chip SRAM structures.
LUTs map multiple input bits to one output bit each (comparable to logic gates) and are wired up with a configurable interconnection network.
The LUT mapping like the interconnection configuration is provided by the programmer.
The reconfigurability aspect of FPGAs allows implementing arbitrary architectures on configuration time, which can be massively parallel.
At the same time, this reconfigurability makes it hard to compare FPGA-based solutions directly.
From a principle point of view, this reconfigurability in the form of so-called soft cores comes at a price: from an efficiency point of view, it is always preferable to implement a module as hard core, being optimized from design to implementation for a specific technology.
However, economic reasons as well as the need to adapt to changes in application behavior often prevent relying solely on hard cores.

Compared to GPUs, FPGAs share the aspects of reduced clock frequency, massive parallelization, and explicit memory hierarchy.
However, FPGAs differ in not being constrained to the use as an accelerator.
Principally they can be deployed anywhere in a compute system.
This in particular is important for concepts like near-data processing or processing on the wire, which allow to substantial reduce the amount of data being moved.
Also, while GPUs excel in floating-point performance, FPGAs rather achieve peak performance for integer-based computations.
As a result, FPGAs are being widely used in various applications, including data centers \cite{conf/isca/PutnamCCCCDEFGGHHHHKLLPPSTXB14}, machine learning \cite{conf/fpga/UmurogluFGBLJV17}, and also data management, which is the focus of this survey.
For database systems specifically they might even outperform GPUs. \cite{conf/norchip/RoozmehL17}
The focus of this survey will thus be FPGA-acceleration of non-relational database systems.

%2. LITERATURE REVIEW (specific statements)
\subsection{Related surveys}

\begin{figure}
    \centering
    \includegraphics[width=0.95\linewidth]{figures/surveys}
    \caption{Existing survey overview and our contribution}
    \label{fig:surveys}
\end{figure}

% Venn diagram
\cref{fig:surveys} shows a Venn diagram of topics related to FPGA-accelerated non-relational database systems. 
In principle there are two main axes of subtopics. 
In light grey we show different kinds of acceleration and in grey we show database system types.
As a secondary axis we also show the popular nonßrelational data models graph, document and key-value in dark grey.
We will discuss first relational database systems from top to bottom and second non-relational database systems from top to bottom.

% Relational
We will not look at non-accelerated relational database surveys, since the field is too broad and not sufficiently relevant to this work.
For FPGA-accelerated relational database systems there has been a recent spike in interest.
In the last two years, there have been three surveys examining the field from different perspectives.
In \cite{journals/dbsk/BecherGBDGMPSTW18}, the authors pose the challenge of using the reconfigurability of the FPGA in relational databases.
This results in open questions on exploitation of heterogeneous hardware, query partitioning and dynamic hardware reconfiguration.
Papaphilippou et al. split up the literature into frameworks (\eg Centaur \cite{conf/fccm/OwaidaSKA17} or DoppioDB \cite{conf/sigmod/SidlerIOKA17}) and specialized accelerators for common operators in a relational database.
They also highlight upcoming technologies for attaching FPGAs to main memory (\ie OpenCAPI) as an important development.
The authors of the most recent survey on the topic \cite{journals/vldb/FangMHLH20} name main memory access, programmability and GPUs as the three biggest factors holding back FPGAs in in-memory relational database systems and how this is being addressed recently, preparing the way for FPGAs as popular accelerators.
Regarding GPU-accelerated relational database systems, the authors of \cite{journals/tlsdkcs/BressHSBS14} raise challenges like the IO bottleneck and query planning, but do not offer convincing solutions.

% Non-relational
The field of non-accelerated non-relational database systems is covered well with surveys and discussed in more detail later in \cref{sec:background}.
Our survey is positioned in the field of FPGA-accelerated non-relational database systems.
To the best of our knowledge there are no surveys on this topic yet, but graph processing on FPGAs as one part of the topic got attention recently. \cite{journals/corr/abs-1903-06697, journals/jcst/Gui0HLCL019}
However, while this shows the feasibilty of graph processing on FPGAs, these surveys are motivated by high performance computing and focus only on the functional aspects of graph processing. 
For our survey this literature has to be viewed from a database standpoint.
We will not revisit GPU acceleration (for graph \cite{journals/csur/ShiZZJHLH18}), because we think they are currently constrained by an IO-bottleneck to the CPU. \cite{journals/tlsdkcs/BressHSBS14}

% Types of database systems not in the figure
Over the history of database systems there was a development from hierarchical/network databases over relational and object-oriented to non-relational database systems and very recently NewSQL database systems. \cite{journals/csur/DavoudianCL18} 
Hierarchical/network and object-oriented database systems have since lost popularity, but the relational and modern non-relational database system literature shows a trend in accelerator usage.
We will not go into more detail of the literature on hierarchical/network, object-oriented and NewSQL database systems.

%3. THE NEED FOR THE PRESENT WORK/Gap (what is missing or wrong in the previous work)

To the best of our knowledge there is no survey on FPGA-accelerated non-relational database systems yet, however the literature and related surveys show the relevance.

%4. OBJECTIVE OF THE PRESENT WORK/Innovation (be specific!)

The objective of this survey is to fill this gap in the intersection of FPGA acceleration and the non-relational data models graph, document and key-value.
We think that looking at graph, document and key-value acceleration and working out differences and commonalities will allow to transfer research between data models and combine multiple data models in one accelerator.
We think that there are overarching patterns and design decisions to find in the literature.

% Research method - probably very important for IS Journal, but not VLDBJ
\subsection{Research method and contributions}

To address this objective, this survey relies on the design science methodology \cite{DBLP:books/sp/Wieringa14} as a rigid method to collect, summarize and evaluate FPGA-accelerated non-relational database solutions.
\Cref{fig:methodology} depicts the research method that we applied, and we used to structure in this paper. On top are the underlying hypotheses and highlighted in grey are the contributions.

\begin{figure*}
    \centering
    \includegraphics[width=0.7\textwidth]{figures/methodology_v3}
    \caption{Research methodology (adapted from \cite{DBLP:books/sp/Wieringa14})}
    % broken, should be: objectives, artifacts, evaluation
    \label{fig:methodology}
\end{figure*}

Our fundamental theory and motivation for this work is: \emph{Existing non-relational databases do not leverage modern FPGA hardware}, from which we derive \textbf{hypothesis (H1)}, i.e.,\ \emph{existing non-relational database systems are not sufficiently FPGA hardware-accelerated}.
This hypothesis is tested based on an introductory system review in \cref{sec:background}.
Further, we belief that this grounds on missing fundamental research on hardware-accelerated non-relational databases (cf. \cref{fig:surveys}), which leads us to \textbf{hypothesis (H2)}, i.e.,\ \emph{current research does not sufficiently address non-relational hardware acceleration}.
We test this hypothesis on another observation artifact, i.e.,\ a systematic literature analysis in \cref{sec:literature}.
The system review aims at analyzing available non-relational database systems regarding relevant aspects and their current state regarding hardware acceleration.
The derived system aspects are then used to guide the systematic literature analysis.
The literature analysis describes, which types of non-relational systems have been previously studied in the context of the aspects and which solutions are provided.
In \textbf{hypothesis (H3)}, we argue that \emph{it is generally unclear how to build a non-relational database with FPGAs}.
To address the detected gaps and missing FPGA-accelerated non-relational database system, we propose new practical pattern categories, on how to build and accelerated non-relational databases or accelerate existing ones.
Finally, resulting open research challenges are described.
This constitutes the following contributions:

\begin{itemize}
    \item System \emph{aspects} resulting from an analysis of existing non-relational database systems and challenges in accelerator design for data-centric applications (\cref{sec:background})
    \item Short paper summaries (\emph{implementations}), aspect reference table and list of \emph{gaps} resulting from a comprehensive literature search along structured design science approach (\cref{sec:literature})
    \item Patternization of literature into \emph{problems}, \emph{placements}, non-trivial accelerator design decisions and accelerated architecture justification as guidelines to system architects (\cref{sec:practitioners_guide})
    \item Open research challenges in the field of FPGA-accelerated non-relational database systems, derived from the gaps in the literature (\cref{sec:challenges})
\end{itemize}

\Cref{sec:summary} will summarize the survey.

%5. (optional) JUSTIFICATION OR IMPORTANCE OF THE PRESENT SUBJECT

%6. (optional) PREVIEW
\subsection{Observations}

In the course of this survey we made the following 5 key observations (highlighted as framed boxes) spanning the three data model types:

\begin{enumerate}
    \item There are three accelerator problem categories (operator, communication layer, and data access acceleration) that FPGAs are currently well suited for, educating the accelerator usage decision.
    \item There are four fundamental patterns of FPGA placement (offload, smart NIC, near-data, and socket).
    \item The data model type in combination with the problem solved by the FPGA are sufficient to define the placement pattern.
    \item Which non-trivial design decisions will become relevant? (\eg for a complete database implementation dynamic queries, design space reduction, memory access are required among other things)
    \item An agreed upon benchmark suite that covers workloads and data sets is missing for robust justification of accelerator usage decisions.
\end{enumerate}

Additionally, the reader will thus learn about the three non-relational database types graph, document, and key-value and how they currently make use of accelerators (\eg scalable key-value solutions were found, but no complete database solution for others).


==> includes/introduction-old.tex <==
\section{Introduction}
\label{sec:introduction}

\todo[inline]{Holger}

% \todo[inline]{Title: \enquote{hardware-acceleration} sounds broad, we only consider \glspl{fpga}; is acceleration or coverage of \gls{fpga} solutions in the focus? \\ $\rightarrow$ (Jonas) The underlying question is: How do/Can we improve qualities (\eg latency, throughput, consistency, scalability or security) of NoSQL databases by adding an \gls{fpga} to the system?}

%%% Motivation / Context

% Motivate NoSQL
In the last few years, NoSQL databases have gained much attention. 
When compared to traditional \glspl{rdbms}, they offer non-relational structuring of data and improved scalability, availability and latency. 
To achieve those properties, they relax traditional database constraints (\eg consistency in PACELC-theorem \cite{journals/computer/Abadi12}). 
Big Data, Internet of Things and other trends benefit greatly from the properties of NoSQL databases and have thus driven a diversification in database systems.

\todo[inline]{variety - data models}

% Differentiate from traditional databases
Despite the name, NoSQL is not defined by the lack of a structured query language (SQL), but rather a new way of thinking about databases. 
Traditionally, databases store data as well formed tables, which impose a structure that is defined at initialization. 
Strong consistency is a key feature of those databases... 
\emph{Irgendwie wiederhole ich mich hier nur. Ich glaube eine Auflistung von key paradigm shifts ist hilfreich}

The key paradigm shifts for NoSQL databases are listed below. 
Those paradigm shifts are freely combineable in an implementation of a NoSQL database. 
NoSQL database features are driven by new requirements in applications. 
Previously there were business applications which required correctness over everything. 
The correctness however imposes a large overhead and centralization that cannot be tolerated in Web $2.0$, Big Data and Internet of Things applications.

Need to \cite{something}:

\begin{enumerate}
    \item Application specific data structure
    \item No/optional schema
    \item Horizontal Scaleability (throughput, replication, partitioning)
    \item Availability
    \item Latency
    \item (Simple API)
\end{enumerate}

\todo[inline]{This is important for the background chapter. What exactly do we want to say here already?}

$\rightarrow$ This leads to data structure relaxation and less consistency

% \todo[inline]{also briefly introduce nosql databases, why are they relevant for our study (and not sql: because there is a lot of literature + references; and differentiate nosql properties from sql, and what will be new in this study); then link to current problems (\eg performance, stability?, different from sql?)}

% Scaling issues of CPU solutions
Motivate why CPU is not sufficient anymore and we need \glspl{fpga}/accelerators in general:

Performance is critical in these systems and CPUs cannot withhold the requirements of ever growing datasets (powerwall not as strong as an argument, because NoSQL databases exhibit better scalability than traditional systems).

% FPGAs can be solution to performance scaling issues
\glspl{fpga} are an upcoming class of accelerators, where earlier restrictions are being addressed \cite{journals/vldb/FangMHLH20}. 
Acceleration with \glspl{fpga} is feasible for problems similar to NoSQL database workloads \cite{journals/corr/abs-1903-06697} (Maybe \glspl{fpga} will work especially well with multi-model, because transformation might be possible on the wire?).

Why do \glspl{gpu} \cite{journals/tlsdkcs/BressHSBS14} not work?

FPGAs can be faster than GPUs for databases: \cite{conf/norchip/RoozmehL17}

%What sets \glspl{fpga} apart:
%\begin{itemize}
%    \item Caching: LRU cache line replacement strategy vs. application specific, Coarse grained cache lines vs. custom cache structure
%    \item Near data processing
%    \item Custom data path on chip
%    \item Massive parallelism
%    \item Low power consumption
%    \item Near network (Zsolt)
%    \item Reconfigurability (against ASICs)
%\end{itemize}

%%% State what was impossible or not satisfactory before the work appeared

To the best of our knowledge there is not survey on improving NoSQL databases by adding FPGAs to the system.

Recent surveys in adjacent fields of research show the relevance of the topic and how timely it is, but do not address FPGAs in NoSQL database systems.

There are surveys on accelerating traditional databases with FPGAs \cite{conf/fpl/PapaphilippouL18, journals/vldb/FangMHLH20, journals/dbsk/BecherGBDGMPSTW18}

There are surveys on NoSQL in general \cite{journals/ife/GessertWFR17, journals/csur/DavoudianCL18, conf/pervasive/HanELD11, GajendranS12, journals/asei/HeC15}

Especially graph processing on FPGAs as one aspect of NoSQL got attention. \cite{journals/corr/abs-1903-06697, journals/jcst/Gui0HLCL019} 
Those surveys are motivated by high performance computing. 
The main weakness is that they focus on the functional aspects.

\begin{figure*}
    \centering
    \includegraphics[width=.75\textwidth]{figures/surveys}
    \caption{Existing survey overview and our contribution}
    \label{fig:surveys}
\end{figure*}

\begin{itemize}
    \item Accelerating database systems using \glspl{fpga}: A survey \cite{conf/fpl/PapaphilippouL18}
    \begin{enumerate}
        \item Challenges: Main memory access and latency
        \item Splits literature into frameworks (Centaur, DoppioDB, ...) and specialized accelerators (sort, selection, join, string matching, filtering, arithmetic)
        \item Also talks about upcoming technologies for attaching FPGA to main memory (OpenCAPI)
    \end{enumerate}
    \item In-memory database acceleration on \glspl{fpga}: a survey \cite{journals/vldb/FangMHLH20}
    \begin{enumerate}
        \item What held back FPGAs (main memory access, programmability, GPUs) and how this is being addressed
        \item Functional aspects: acceleration of different query operators (streaming, decompression, sorting, join, partitioning)
        \item Future research questions: database architecture with multiple different computational elements in mind, accelerator design, comparison with GPUs, compilation for FPGAs
    \end{enumerate}
    \item Integration of \glspl{fpga} in Database Management Systems: Challenges and Opportunities \cite{journals/dbsk/BecherGBDGMPSTW18}
    \begin{enumerate}
        \item Integration of a FPGA into a DB, with consideration of reconfigurability
        \item Resulting challenges: exploitation of heterogeneous hardware, query partitioning, dynamic hardware reconfiguration
    \end{enumerate}
    \item NoSQL database systems: a survey and decision guidance \cite{journals/ife/GessertWFR17}
    \begin{enumerate}
        \item Key-value, document, wide-column
        \item ``Comparative classification model that relates functional and non-functional requirements to techniques and algorithms employed in NoSQL databases''
    \end{enumerate}
    \item A Survey on NoSQL Stores \cite{journals/csur/DavoudianCL18}
    \begin{enumerate}
        \item Strong start with timeline
        \item Key-value, wide-column, document, graph
        \item Main aspects are consistency, partitioning and CAP
    \end{enumerate}
    \item Survey on NoSQL Database \cite{conf/pervasive/HanELD11}
    \begin{enumerate}
        \item Key-value, wide-column, document
        \item CAP
    \end{enumerate}
    \item A Survey on NoSQL Databases \cite{GajendranS12}
    \begin{enumerate}
        \item Key-value, wide-column, document
    \end{enumerate}
    \item Survey on NoSQL database technology \cite{journals/asei/HeC15}
    \begin{enumerate}
        \item Key-value, wide-column, document, graph
    \end{enumerate}
    \item Graph Processing on \glspl{fpga}: Taxonomy, Survey, Challenges \cite{journals/corr/abs-1903-06697}
    \item A Survey on Graph Processing Accelerators: Challenges and Opportunities \cite{journals/jcst/Gui0HLCL019}
    \begin{enumerate}
        \item CPU: low efficiency (irregularities do not exploit memory- and instruction-level parallelism)
        \item GPUs: control and memory divergence, load imbalance, unnecessary global memory accesses
        \item Preprocessing, parallel graph computation, runtime scheduling
        \item Major challenge: programmability
        \item Comprehensive list of algorithms
    \end{enumerate}
    \item GPU-Accelerated Database Systems: Survey and Open Challenges \cite{conf/adbis/BressHSBS13} \cite{journals/tlsdkcs/BressHSBS14}
    \item GraphProcessing on GPUs: A Survey \cite{journals/csur/ShiZZJHLH18}
    %\item Big Data Analytics on Modern Hardware Architectures: A Technology Survey \cite{conf/ebiss/SaeckerM12}
\end{itemize}

% Differentiate our survey from existing ones
We look at aspects specific to NoSQL databases on FPGAs (More specific than HPC graph processing, in-memory database on FPGAs, NoSQL in general, ...).

There is a lack of looking at the non-functional aspects.

%%% What are the challenges in the area of this work?

%What is the challenge we address?
Create a catalogue of solutions to problems in integrating FPGAs into NoSQL databases and develop a vision for future hardware-accelerated NoSQL databases. 
Open challenges/gap

%%% What is the idea of the solution? How do we address the challenges better than before?

\todo[inline]{methodology}

We do an extensive literature search, but there is almost no literature specific to integrating an \glspl{fpga} in the context of a NoSQL database. 
Thus, we query adjacent fields of research and create transferable solutions.

Motivate the domains we have chosen (missing are e.g. time series, object oriented, scientific). 
The same domains plus wide-column stores can be found in NoSQL surveys. 
Out of scope

While not the defining factor of NoSQL, databases in the field are mainly categorized by the structure of the data they store. 
The most important data structures are graphs, geospatial geometries, documents and key-value pairs. 
Those four categories will be the focus of this survey. 
Other data structures are \eg time series or objects. 
Recently, there has been a trend to collapse concepts in different kinds of NoSQL databases to form multi-model databases.

\todo[inline]{out of scope + rationale; NoSQL: no RDF, tuple-stores; no NewSQL, object-oriented dbs, network, relational}

Multi-model?

% Research method - probably very important for IS Journal, but not VLDBJ
\subsection{Research method}
This survey relies on the design science methodology \cite{DBLP:books/sp/Wieringa14} as a rigid method to collect, summarize and evaluate FPGA-accelerated NoSQL database solutions.
\Cref{todo} depicts the research method that we applied, and we used to structure in this paper.

Our fundamental theory and motivation for this work is: \emph{Existing NoSQL databases do not leverage modern FPGA hardware}, from which we derive \textbf{hypothesis (H1)}, i.e.,\ \emph{existing NoSQL systems are not sufficiently FPGA hardware-accelerated}.
This hypothesis is tested based on an introductory system review in \cref{sec:background}.
Further, we belief that this grounds on missing fundamental research on hardware-accelerated NoSQL databases (cf. \cref{fig:surveys}), which leads us to \textbf{hypothesis (H2)}, i.e.,\ \emph{current research does not sufficiently address NoSQL hardware acceleration}.
We test this hypothesis on another observation artifact, i.e.,\ a systematic literature review in \cref{sec:literature}.
The system review aims at analyzing available NoSQL systems regarding relevant NoSQL system aspects components / architecture and their current state regarding hardware acceleration.
The derived system aspects are then used to guide the systematic literature review.
The review analyses, which types of NoSQL system types have been previously studied in the context of the system aspects and which solutions are provided.
In \textbf{hypothesis (H3)}, we argue that \emph{it is generally unclear how to build or accelerate a NoSQL database with FPGAs}.
To address the detected gaps and missing FPGA-accelerated NoSQL system, we propose new practical pattern categories, on how to build and accelerated NoSQL database or accelerate and existing one.
Finally, resulting research directions are described.

% Outline
%%% Contributions of this work and outline
\subsection{Contributions and paper outline}

This paper makes the following contributions:
\begin{itemize}
    \item Analysis of existing NoSQL database systems and trends in the field ($\rightarrow$ H1),
    \item Comprehensive literature search along structured design science approach resulting in reference list and short paper summaries ($\rightarrow$ H2),
    \item Patternization of literature into placement, performance and application view as guidelines to system builders on different aspects ($\rightarrow$ H3).
\end{itemize}

The paper is structured as follows. \todo[inline]{outline}
